Tokenization Repair in the Presence of Spelling Errors

We consider the following tokenization repair problem: Given a natural language text with any combination of missing or spurious spaces, correct these. Spelling errors can be present, but it's not part of the problem to correct them. For example, given: "Tispa per isabout token izaionrep air", compute "Tis paper is about tokenizaion repair". We identify three key ingredients of high-quality tokenization repair, all missing from previous work: deep language models with a bidirectional component, training the models on text with spelling errors, and making use of the space information already present. Our methods also improve existing spell checkers by fixing not only more tokenization errors but also more spelling errors: once it is clear which characters form a word, it is much easier for them to figure out the correct word. We provide six benchmarks that cover three use cases (OCR errors, text extraction from PDF, human errors) and the cases of partially correct space information and all spaces missing. We evaluate our methods against the best existing methods and a non-trivial baseline. We provide full reproducibility under https://ad.cs.uni-freiburg.de/publications .

==> figures/bidirectional_lms.tex <==

\begin{figure*}[bt]
    \begin{subfigure}{0.5\textwidth}
        \begin{center}
            \scalebox{0.9}{
                \begin{tikzpicture}

                    \node[minimum size=1em] (x0) at (0*\xoffset, -0.25){...};
                    \node[minimum size=1em] (x1) at (1*\xoffset, -0.25){$b$};
                    \node[minimum size=1em] (x2) at (2*\xoffset, -0.25){$\mathit{space}$};
                    \node[minimum size=1em] (x3) at (3*\xoffset, -0.25){$a$};
                    \node[minimum size=1em] (x4) at (4*\xoffset, -0.25){...};

                    \node[minimum size=\boxsize] (fwd0) at (0*\xoffset, 1){...};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (fwd1) at (1*\xoffset, 1){$\mathrm{LSTM}_f$};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (fwd2) at (2*\xoffset, 1){$\mathrm{LSTM}_f$};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (fwd3) at (3*\xoffset, 1){$\mathrm{LSTM}_f$};
                    \node[minimum size=\boxsize] (fwd4) at (4*\xoffset, 1){...};
                    
                    \node[minimum size=\boxsize] (bwd0) at (0*\xoffset, 2.5){...};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (bwd1) at (1*\xoffset, 2.5){$\mathrm{LSTM}_b$};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (bwd2) at (2*\xoffset, 2.5){$\mathrm{LSTM}_b$};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (bwd3) at (3*\xoffset, 2.5){$\mathrm{LSTM}_b$};
                    \node[minimum size=\boxsize] (bwd4) at (4*\xoffset, 2.5){...};

                    \node[minimum size=\boxsize] (fc1) at (1*\xoffset, 4){...};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (fc2) at (2*\xoffset, 4){FC};
                    \node[minimum size=\boxsize] (fc3) at (3*\xoffset, 4){...};
                    
                    \node[minimum size=\boxsize] (out1) at (1*\xoffset, 5.5){...};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (out2) at (2*\xoffset, 5.5){output};
                    \node[minimum size=\boxsize] (out3) at (3*\xoffset, 5.5){...};
                    
                    \node[minimum size=\boxsize] (y1) at (1*\xoffset, 6.75){...};
                    \node[minimum size=1em] (y2) at (2*\xoffset, 6.75){$p_\mathit{bi}(c|c_b, c_a)$};
                    \node[minimum size=\boxsize] (y3) at (3*\xoffset, 6.75){...};
                    
                    \draw[->] (x1) -> (fwd1);
                    \draw[->] (x2) -> (fwd2);
                    \draw[->] (x3) -> (fwd3);
                    
                    \draw[->] (x1) to[bend left] (bwd1.south);
                    \draw[->] (x2) to[bend left] (bwd2.south);
                    \draw[->] (x3) to[bend left] (bwd3.south);
                    
                    \draw[->] (fwd0) -> (fwd1);
                    \draw[->] (fwd1) -> (fwd2);
                    \draw[->] (fwd2) -> (fwd3);
                    \draw[->] (fwd3) -> (fwd4);
                    
                    \draw[->] (bwd4) -> (bwd3);
                    \draw[->] (bwd3) -> (bwd2);
                    \draw[->] (bwd2) -> (bwd1);
                    \draw[->] (bwd1) -> (bwd0);
                    
                    \draw[->] (fwd1.north) -> (fc2.south);
                    \draw[->] (bwd3.north) -> (fc2.south);
                    
                    \draw[->] (fc2) -> (out2);
                    
                    \draw[->] (out2) -> (y2);
                \end{tikzpicture}
            }
            \caption{character probability estimation}
            \label{subfig:prediction}
        \end{center}
    \end{subfigure}
    \begin{subfigure}{0.5\textwidth}
        \begin{center}
        \scalebox{0.9}{
            \begin{tikzpicture}
                    \node[minimum size=1em] (x0) at (0*\xoffset, -0.25){...};
                    \node[minimum size=1em] (x1) at (1*\xoffset, -0.25){$b$};
                    \node[minimum size=1em] (x3) at (2*\xoffset, -0.25){$a$};
                    \node[minimum size=1em] (x4) at (3*\xoffset, -0.25){...};

                    \node[minimum size=\boxsize] (fwd0) at (0*\xoffset, 1){...};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (fwd1) at (1*\xoffset, 1){$\mathrm{LSTM}_f$};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (fwd2) at (2*\xoffset, 1){$\mathrm{LSTM}_f$};
                    \node[minimum size=\boxsize] (fwd4) at (3*\xoffset, 1){...};
                    
                    \node[minimum size=\boxsize] (bwd0) at (0*\xoffset, 2.5){...};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (bwd1) at (1*\xoffset, 2.5){$\mathrm{LSTM}_b$};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (bwd2) at (2*\xoffset, 2.5){$\mathrm{LSTM}_b$};
                    \node[minimum size=\boxsize] (bwd4) at (3*\xoffset, 2.5){...};

                    \node[minimum size=\boxsize] (fc1) at (0.5*\xoffset, 4){...};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (fc2) at (1.5*\xoffset, 4){FC};
                    \node[minimum size=\boxsize] (fc3) at (2.5*\xoffset, 4){...};
                    
                    \node[minimum size=\boxsize] (out1) at (0.5*\xoffset, 5.5){...};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (out2) at (1.5*\xoffset, 5.5){output};
                    \node[minimum size=\boxsize] (out3) at (2.5*\xoffset, 5.5){...};
                    
                    \node[minimum size=\boxsize] (y1) at (0.5*\xoffset, 6.75){...};
                    \node[minimum size=1em] (y2) at (1.5*\xoffset, 6.75){$p_\mathit{bi}(c|c_b, c_a)$};
                    \node[minimum size=\boxsize] (y3) at (2.5*\xoffset, 6.75){...};
                    
                    \draw[->] (x1) -> (fwd1);
                    \draw[->] (x2) -> (fwd2);
                    
                    \draw[->] (x1) to[bend left] (bwd1.south);
                    \draw[->] (x2) to[bend left] (bwd2.south);
                    
                    \draw[->] (fwd0) -> (fwd1);
                    \draw[->] (fwd1) -> (fwd2);
                    \draw[->] (fwd2) -> (fwd3);
                    
                    \draw[->] (bwd3) -> (bwd2);
                    \draw[->] (bwd2) -> (bwd1);
                    \draw[->] (bwd1) -> (bwd0);
                    
                    \draw[->] (fwd1.north) -> (fc2.south);
                    \draw[->] (bwd2.north) -> (fc2.south);
                    
                    \draw[->] (fc2) -> (out2);
                    
                    \draw[->] (out2) -> (y2);
                \end{tikzpicture}
        }
        \caption{insertion probability estimation}
        \label{subfig:insertion}
        \end{center}
    \end{subfigure}
    
    \caption{Bidirectional model.}
    \label{fig:bidirectional}
\end{figure*}


==> figures/unidirectional_lms.tex <==


\newcommand{\xoffset}{1.5}
\newcommand{\boxsize}{3.5em}

\begin{figure*}[bt]
    \begin{subfigure}{0.5\textwidth}
        \begin{center}
            \scalebox{0.9}{
                \begin{tikzpicture}

                    \node[minimum size=1em] (x0) at (0*\xoffset, -0.25){SOS};
                    \node[minimum size=1em] (x1) at (1*\xoffset, -0.25){H};
                    \node[minimum size=1em] (x2) at (2*\xoffset, -0.25){e};
                    \node[minimum size=1em] (x3) at (3*\xoffset, -0.25){l};
                    \node[minimum size=1em] (x4) at (4*\xoffset, -0.25){l};
                    \node[minimum size=1em] (x5) at (5*\xoffset, -0.25){o};

                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (rnn0) at (0*\xoffset, 1){LSTM};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (rnn1) at (1*\xoffset, 1){LSTM};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (rnn2) at (2*\xoffset, 1){LSTM};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (rnn3) at (3*\xoffset, 1){LSTM};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (rnn4) at (4*\xoffset, 1){LSTM};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (rnn5) at (5*\xoffset, 1){LSTM};

                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (fc0) at (0*\xoffset, 2.5){FC};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (fc1) at (1*\xoffset, 2.5){FC};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (fc2) at (2*\xoffset, 2.5){FC};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (fc3) at (3*\xoffset, 2.5){FC};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (fc4) at (4*\xoffset, 2.5){FC};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (fc5) at (5*\xoffset, 2.5){FC};
                    
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (out0) at (0*\xoffset, 4){output};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (out1) at (1*\xoffset, 4){output};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (out2) at (2*\xoffset, 4){output};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (out3) at (3*\xoffset, 4){output};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (out4) at (4*\xoffset, 4){output};
                    \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (out5) at (5*\xoffset, 4){output};
                    
                    \node[minimum size=1em] (y0) at (0*\xoffset, 5.25){$p_f(c|'')$};
                    \node[minimum size=1em] (y1) at (1*\xoffset, 5.25){$p_f(c|S_{1})$};
                    \node[minimum size=1em] (y2) at (2*\xoffset, 5.25){$p_f(c|S_{1:2})$};
                    \node[minimum size=1em] (y3) at (3*\xoffset, 5.25){$p_f(c|S_{1:3})$};
                    \node[minimum size=1em] (y4) at (4*\xoffset, 5.25){$p_f(c|S_{1:4})$};
                    \node[minimum size=1em] (y5) at (5*\xoffset, 5.25){$p_f(c|S_{1:5})$};

                    \draw[->] (x0) -> (rnn0);
                    \draw[->] (x1) -> (rnn1);
                    \draw[->] (x2) -> (rnn2);
                    \draw[->] (x3) -> (rnn3);
                    \draw[->] (x4) -> (rnn4);
                    \draw[->] (x5) -> (rnn5);
                
                    \draw[->] (rnn0) -> (rnn1);
                    \draw[->] (rnn1) -> (rnn2);
                    \draw[->] (rnn2) -> (rnn3);
                    \draw[->] (rnn3) -> (rnn4);
                    \draw[->] (rnn4) -> (rnn5);
                    
                    \draw[->] (rnn0) -> (fc0);
                    \draw[->] (rnn1) -> (fc1);
                    \draw[->] (rnn2) -> (fc2);
                    \draw[->] (rnn3) -> (fc3);
                    \draw[->] (rnn4) -> (fc4);
                    \draw[->] (rnn5) -> (fc5);
                    
                    \draw[->] (fc0) -> (out0);
                    \draw[->] (fc1) -> (out1);
                    \draw[->] (fc2) -> (out2);
                    \draw[->] (fc3) -> (out3);
                    \draw[->] (fc4) -> (out4);
                    \draw[->] (fc5) -> (out5);
                    
                    \draw[->] (out0) -> (y0);
                    \draw[->] (out1) -> (y1);
                    \draw[->] (out2) -> (y2);
                    \draw[->] (out3) -> (y3);
                    \draw[->] (out4) -> (y4);
                    \draw[->] (out5) -> (y5);

                \end{tikzpicture}
            }
            \caption{forward model}
        \end{center}
    \end{subfigure}
    \begin{subfigure}{0.5\textwidth}
        \begin{center}
        \scalebox{0.9}{
            \begin{tikzpicture}

                \node[minimum size=1em] (x0) at (0*\xoffset, -0.25){EOS};
                \node[minimum size=1em] (x1) at (1*\xoffset, -0.25){o};
                \node[minimum size=1em] (x2) at (2*\xoffset, -0.25){l};
                \node[minimum size=1em] (x3) at (3*\xoffset, -0.25){l};
                \node[minimum size=1em] (x4) at (4*\xoffset, -0.25){e};
                \node[minimum size=1em] (x5) at (5*\xoffset, -0.25){H};

                \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (rnn0) at (0*\xoffset, 1){LSTM};
                \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (rnn1) at (1*\xoffset, 1){LSTM};
                \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (rnn2) at (2*\xoffset, 1){LSTM};
                \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (rnn3) at (3*\xoffset, 1){LSTM};
                \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (rnn4) at (4*\xoffset, 1){LSTM};
                \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (rnn5) at (5*\xoffset, 1){LSTM};

                \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (fc0) at (0*\xoffset, 2.5){FC};
                \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (fc1) at (1*\xoffset, 2.5){FC};
                \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (fc2) at (2*\xoffset, 2.5){FC};
                \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (fc3) at (3*\xoffset, 2.5){FC};
                \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (fc4) at (4*\xoffset, 2.5){FC};
                \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (fc5) at (5*\xoffset, 2.5){FC};
                
                \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (out0) at (0*\xoffset, 4){output};
                \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (out1) at (1*\xoffset, 4){output};
                \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (out2) at (2*\xoffset, 4){output};
                \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (out3) at (3*\xoffset, 4){output};
                \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (out4) at (4*\xoffset, 4){output};
                \node[minimum size=\boxsize,fill=gray!10,rectangle,draw] (out5) at (5*\xoffset, 4){output};
                
                \node[minimum size=1em] (y0) at (0*\xoffset, 5.25){$p_b(c|'')$};
                \node[minimum size=1em] (y1) at (1*\xoffset, 5.25){$p_b(c|S_5)$};
                \node[minimum size=1em] (y2) at (2*\xoffset, 5.25){$p_b(c|S_{5:4})$};
                \node[minimum size=1em] (y3) at (3*\xoffset, 5.25){$p_b(c|S_{5:3})$};
                \node[minimum size=1em] (y4) at (4*\xoffset, 5.25){$p_b(c|S_{5:2})$};
                \node[minimum size=1em] (y5) at (5*\xoffset, 5.25){$p_v(c|S_{5:1})$};

                \draw[->] (x0) -> (rnn0);
                \draw[->] (x1) -> (rnn1);
                \draw[->] (x2) -> (rnn2);
                \draw[->] (x3) -> (rnn3);
                \draw[->] (x4) -> (rnn4);
                \draw[->] (x5) -> (rnn5);
            
                \draw[->] (rnn0) -> (rnn1);
                \draw[->] (rnn1) -> (rnn2);
                \draw[->] (rnn2) -> (rnn3);
                \draw[->] (rnn3) -> (rnn4);
                \draw[->] (rnn4) -> (rnn5);
                
                \draw[->] (rnn0) -> (fc0);
                \draw[->] (rnn1) -> (fc1);
                \draw[->] (rnn2) -> (fc2);
                \draw[->] (rnn3) -> (fc3);
                \draw[->] (rnn4) -> (fc4);
                \draw[->] (rnn5) -> (fc5);
                
                \draw[->] (fc0) -> (out0);
                \draw[->] (fc1) -> (out1);
                \draw[->] (fc2) -> (out2);
                \draw[->] (fc3) -> (out3);
                \draw[->] (fc4) -> (out4);
                \draw[->] (fc5) -> (out5);
                
                \draw[->] (out0) -> (y0);
                \draw[->] (out1) -> (y1);
                \draw[->] (out2) -> (y2);
                \draw[->] (out3) -> (y3);
                \draw[->] (out4) -> (y4);
                \draw[->] (out5) -> (y5);

            \end{tikzpicture}
        }
        \caption{backward model}
        \end{center}
    \end{subfigure}
    
    \caption{The unidirectional models predicting the example sequence $S$ = ``Hello''.
             The LSTM, FC and output boxes always refer to the same LSTM cell, fully connected layer and output layer in a model.
             SOS and EOS are special symbols marking the beginning and end of a sequence.}
    \label{fig:unidirectional}
\end{figure*}


==> sections/deprecated.tex <==
\iffalse
\begin{table}[!h]
\centering
\renewcommand{\baselinestretch}{1.2}\small
\begin{tabular}{|l|c|c|c|}\hline
Type          & Freq. & Prediction& Ground T. \\ \hline
Compounds     & 29\% & `box set' & `boxset' \\
Foreign       &21\% & `De Clercq' & `DeClercq'\\
Entities      & 19\%  & `First Energy' & `FirstEnergy'\\
Punctuation   &19\% & `(March)' & `( March )'\\
Measurements  &8\% & `10 m' & `10m' \\
Abbreviations &2\% & `K. K.' & `K.K.' \\
Unk. alphabet &2\% & &\\ %\eg unknown foreign alphabet. & & \\
\hline
\end{tabular}
\caption{Error analysis of beam search bidirectional model.
    Splitting/merging compound words is the most common error, inclduing
    entity names (\eg companies).
    Near foreign names/words is the next category.
    The remaining categories are near measurements, abbreviations,unknown alphabet,
    and ambiguities in ground truth near punctuations.
    }
\label{tab:errors-bidir}
\vspace{-0.5cm}
\end{table}
\fi


\iffalse
We examined a sample of \TODO{100} wrong predictions of our \TODO{approaches},
and it turned out to be that, many of them are especially difficult cases, categorized as follows:
\begin{itemize}[wide, labelwidth=!, labelindent=0pt, noitemsep, topsep=0pt]
    \item Technical terms \begin{center}`KTMRC 390' instead of `KTM RC390'\end{center}
    \item False split of compound words `northeastern'
    \item Missing split of compound words `crewman'
    \item He/she ambiguity `setbacks he' vs. `setback she'
    \item Foreign language
        \begin{center} `Iusabutendi' instead of `Ius abutendi' \\ `rotundi maxillaris' instead of `rotundimaxillaris' \end{center}
    \item False split of names `Es the fanny' instead of `Esthefanny'
    \item Missing space of names `Sanovaan' instead of `Sano vaan'.
    \item Punctuation inconsistency, `todo :' vs. `todo:'
    \item Ground truth inconsistency \TODO{explain}
    \item \TODO{missing typos errors}
\end{itemize}
\fi
%Some cases are ambiguous, in the sense that both alternatives - with and without space - appear in the training data (for example ``script writer'' and ``scriptwriter'').
%Some errors result from CamelCase names that get split by our approaches.
%Few cases require an understanding of the sentence to be correctly predicted.
%For example, to distinguish between ``votes he received'' and ``vote she received'' requires knowledge of whether the person who was mentioned before is considered male or female.

%We find that some cases can not be predicted correctly, because the tokenization in the ground truth sequences is inconsistent or erroneous.
%More unsolvable cases arise with the introduction of misspellings.
%For example, when a typo inserts a random character at the beginning or end of
%a token, it is unclear whether the character belongs to the left or right
%token, and our approaches sometimes isolate it to a single-character word.


%\subsubsection{Failed attempts}

%Another early attempt using iterative correcting procedure was done. This was 
%processing the sequence and fixing tokenization errors that are not too near, then
%iteratively repeats the process until it fixes all errors. This turned out to be
%disadvantageous, because the models needed careful thersholding strategy to decide
%where to make a fix, which turned out to be inferior in our experiments.
%Moreover, their runtime was much slower than beam search, because they strongly
%depended on the number of tokenization errors, while the beam search doesn't.

\iffalse
\begin{table*}[htb]
 \renewcommand{\baselinestretch}{1.2}\small
 \begin{center}
  \begin{tabular}{|l|cccc|cccc|cccc|}
   \hline
               & \multicolumn{4}{c|}{10\,\%} & \multicolumn{4}{c|}{100\,\%} & \multicolumn{4}{c|}{no \msp} \\
   Approach    & Fc    & Fs    & F     & Acc.  & Fc    & Fs    & F     & Acc.  & Fc    & Fs    & F     & Acc.  \\
   \hline
   Google      & 60.2  & 83.3  & 70.7  & 43.0  & 26.9  & 53.6  & 47.3  &  7.0  &  2.5  & 15.0  & 13.8  & 10.0  \\
   beam search & 79.0  & 96.6  & 88.0  & 67.1  & 87.4  & 98.9  & 96.7  & 63.1  & 75.3  & 98.7  & 96.7  & 62.4  \\
   \hline
  \end{tabular}
  \caption{Spelling correction evaluation. All values in per cent. Fc is the F-score on character edits, Fs on space edits, F on all edits. Acc is the sequence accuracy.}
 \end{center}
\end{table*}
\fi


\iffalse
\subsubsection{Dynamic programming (``DP fixer'')}
The dynamic programming baseline attempts to fix the tokenization of a text $S$, 
by retokenizing the non-space characters in $S$ in a top-down divide-and-conquer approach.
This is done by deciding to insert or not to insert spaces between
all non-space characters in the given sequence, in a manner that after retokenization, all the words should be
correct as identified by a reference words dictionary $D$.  
Given a word $w$ consisting of non-space characters, we can attempt to 
choose the first word $w_{[i, j^{*})}$ (for some optimal $j^{*}$) and score it according to a
scoring function $Q$ then retokenize the remaining word recursively,
using the optimization formula:
$$R(w, i) = \max_{i < j \leq |w|} Q_D(w_{[i, j)}) + R(w, j)$$
where $Q$ is the scoring function, defined by:
$$Q_D(w) = \begin{cases} (\alpha |w|^2 + \beta |w| + 1) \gamma^{e_D(w)} & \text{ if } e \leq 1 \\ 0 & \text{otherwise}\end{cases}$$
where $\alpha=1.15, \beta=0.1, \gamma=0.5$ are fixed parameters and $e_D( w)$
is the edit distance to the closest word in the dictionary.
After the initial formula $R(w, 0)$ is computed, the traceback of the recursion can be
used to construct the retokenized fixed sentence.

The dictionary is implemented using the Trie data structure \cite{trie} to be efficient
in search including minor typos.
The damping factor $\gamma$ is needed to be more robust in case of typos
or non-existing words in the dictionary.
Additionally, the scoring function needs to have combinations of $|w|, |w|^2$,
because only the constant terms will prefer to break a word like `impatient' to `im' and `patient', because
`im' partially matches with `in', and `patient' fully matches, which would be higher than one full match `impatient'.
Also, the quadratic term prefers longer words, so the algorithm doesn't end up
retokenizing `however' into `how', `ever'. The values of $\alpha, \beta, \gamma$ were
found through experimentation on small set of examples.
Finally, to reduce the time complexity of the function $R$, we restrict the usage of 
$R$ to be only on windows of small size $W$ tokens ($W=5$ in our experiments),
so it will try to retokenize only nearby tokens.

\label{subsec:dp}

\subsection{Enchant}

We use the Enchant spell checker\footnote{\url{https://abiword.github.io/enchant}}
with the GNU Aspell\footnote{\url{http://aspell.net}} backend
to test the performance of an open source spell checker on tokenization repair.
We replace a word when the spell checker suggests a split as a correction.
Merging words is not supported by the spell checker.
\fi



\iffalse
\subsubsection{Iterative correction}

The first correction approach is to iteratively insert and delete spaces where the combined or bidirectional model gives a high probability.

\paragraph{Algorithm:}
All space deletion probabilites $p_\del$ and space insertion probabilities $p_\ins$ are estimated
and compared to threshold values $t_\del$ and $t_\ins$:
\begin{center}
 $\mathit{score}_\ins = (p_\ins - t_\ins) / (1 - t_\ins)$\\
 $\mathit{score}_\del = (p_\del - t_\del) / (1 - t_\del)$
\end{center}
All space insertions and deletions with a positive score are executed, if no other insertion or deletion in a window of 10 characters to the left and right has a greater score.
Then, the next iteration starts with re-estimating the space insertion and deletion probabilities on the edited sequence.
The procedure stops when no more insertion or deletion operation has a positive score.

\paragraph{Threshold optimization:}
The values for $t_\ins$ and $t_\del$ are tuned on a development set of sequences with corrupt tokenization.
The probability for every possible space insertion and deletion is estimated on the sequence where all other characters are correct, and the thresholds are set such that the F-score of all edits with probabilities above the threshold is maximized.
A definition of the F-score is given in section \ref{sec:evaluations:metrics}.


\fi

\iffalse
\paragraph{Combined model:}
The forward model and backward model are combined into a single model.
The combination is done by multiplying the probabilities estimated by the
two models and normalizing over all possible characters:
$$p_\bi(s|c_b, c_a) = \frac{p_f(s|c_b) p_b(s|c_a)}
{\sum_{s' \in V} p_f(s'|c_b) p_b(s'|c_a)}\,$$

The space insertion probability is computed by comparing the space probability
with the probabilities of the first character $a$ of $c_a$ and the last character $b$ of $c_b$:
$$p_\ins(c_b, c_a) = \frac{p_f(\msp|c_b) p_b(\msp|c_a)}
{p_f(\msp|c_b) p_b(\msp|c_a) + p_f(a|c_b) p_b(b|c_a)}\,$$

The space deletion probability is the inverse of the space insertion probability:
$$p_\del(c_b, c_a) = \frac{p_f(a|c_b) p_b(b|c_a)}
{p_f(\msp|c_b) p_b(\msp|c_a) + p_f(a|c_b) p_b(b|c_a)}\,$$


\paragraph{Bidirectional model:}
The bidirectional model estimates $p_\bi(s | \allowbreak c_b, c_a)$ directly.
It consists of a forward and a backward LSTM cell of 1024 units.
To estimate the probability $p_\bi(s_i|c_b, c_a)$,
the outputs of the forward cell after processing $s_{i-1}$
and the backward cell after processing $s_{i+1}$ are fed into a dense layer,
which is followed by a classification output layer.
With a softmax output function the model tended to insert spaces at wrong positions.
We therefore use a sigmoid output function, so that the model can predict the absence of any character between two contexts by predicting the 0 vector.

The space deletion probability is computed as the inverse space probability:
\begin{center}
 $p_\del(c_b, c_a) = 1 - p_\bi(\msp|c_b, c_a)$
\end{center}
To estimate insertion probabilities $p_\ins^\bi(s|c_b, c_a)$
between two characters $s_i$ and $s_{i+1}$,
the outputs of the forward cell after $s_{i}$
and the backward cell after $s_{i+1}$ are fed into the dense layer.
\begin{center}
 $p_\ins(c_b, c_a) = p_\ins^\bi(\msp|c_b, c_a)\,.$
\end{center}

The model was trained by minimizing the sum of two losses:
the binary crossentropy of the characters in the training sequences
and the binary crossentropy of the predicted insertion probabilities compared with the zero vector.
\fi



\iffalse
Table \ref{tab:datasets} gives more statistics of the dataset.

\begin{table}[t]
\begin{center}
\renewcommand{\baselinestretch}{1.15}\normalsize
\begin{tabular}{|l|c|}\hline
    Measure                      &  Value          \\ \hline
    Number of documents          &      5,880,206  \\
    Number of sequences          &     43,250,909  \\
    Number of tokens             &  2,107,696,872  \\
    Number of characters         & 12,900,540,122  \\
    Mean tokens per sequence     &           48.7  \\
    Mean characters per sequence &          298.3  \\
    Unique words                 &      6,903,307  \\
    Unique characters            &         17,748  \\
    Size                         &       12.97 GB  \\
\hline
\end{tabular}
    \caption{Statistics of the Wikipedia dataset before splitting it into test, development and training sets.
    We define tokens to be subsequences separated by spaces,
    whereas words are defined as maximal alphanumeric subsequences.
    \TODO{Is there a particular difference between token and word?}
    }
\label{tab:datasets}
\end{center}
\end{table}
\fi

\iffalse
\subsubsection{Deep learning metrics}

\textbf{Accuracy}. The accuracy measures how many examples are classified correctly. 
\\\\
\textbf{Top-$n$ accuracy}. The top-$n$ accuracy measures how many examples have the correct
class classified in the top $n$ predicted classes.
\\\\
\textbf{Categorical crossentropy}.
$$\mathcal{L}(y, \hat{y}) = -\frac{1}{N} \sum_{i=1}^N \sum_c {y^{(i)}_c \log \hat{y}^{(i)}_c}$$
\fi

\iffalse
\\\\
\textbf{Precision}.
%%%$$\mathit{precision}(T, C, F) = \frac{ |\mathcal{C} \setminus \mathcal{F}| }{ |\mathcal{C} \setminus \mathcal{F}| + |\mathcal{F} \setminus \mathcal{C}| }$$
$$\mathit{P}(T, C, F) = \frac{ |\mathcal{C}| - |\mathcal{C} \cap\mathcal{F}| }{ |\mathcal{C}| + |\mathcal{F}| - 2 |\mathcal{C} \cap \mathcal{F}|} $$
\\\\
\textbf{Recall}.
%%%$$\mathit{recall}(T, C, F) = \frac{ |\mathcal{C} \setminus \mathcal{F}| }{ |\mathcal{C}| }$$
$$\mathit{R}(T, C, F) = \frac{ |\mathcal{C}| - |\mathcal{C} \cap \mathcal{F}| }{ |\mathcal{C}| }$$
\fi

\iffalse
\begin{table}[htb]
\begin{center}
\renewcommand{\baselinestretch}{1.15}\normalsize
\begin{tabular}{|l|c|c|c|c|} \hline
Model          & Precision  & Recall    & F-score     \\ \hline
forward        & 84.96\,\%  & 93.88\,\% & 89.20\,\%   \\
backward       & 94.32\,\%  & 97.41\,\% & 95.84\,\%   \\
combined       & 98.04\,\%  & 99.73\,\% & 98.88\,\%   \\
bidir. softmax & 99.38\,\%  & 99.71\,\% & 99.55\,\%   \\
bidir. sigmoid & 99.32\,\%  & 99.70\,\% & 99.51\,\%   \\
%\begin{tabular}{|l|c|c|c|c|} \hline
%Model           & Acc & Top-5 acc  & Cat.CE \\ \hline
%forward         & 71.30\,\% & 90.47\,\%  & 0.963   \\
%backward        & 70.81\,\% & 90.56\,\%  & 0.974   \\
%combined        & 90.61\,\% & 97.03\,\%  & 0.323   \\
%bidir. softmax  & 95.51\,\% & 98.98\,\%  & 0.149   \\
%bidir. sigmoid  & 94.93\,\% & 98.59\,\%  & -       \\
\hline
\end{tabular}
\caption{The language models evaluated on the prediction of spaces on the development sequences.
\textit{Precision} is the fraction of correct predictions among the predicted spaces.
\textit{Recall} is the fraction of true spaces that the model predicts.
\textit{F-score} is the harmonic mean of precision and recall.}
\label{tab:spaceresults}
\end{center}
\end{table}
\fi

\iffalse
%\iffalse
\begin{table}[htb]
 \begin{center}
 \begin{tabular}{|l|cc|cc|}
  \hline
    & \multicolumn{2}{c|}{no typos} & \multicolumn{2}{c|}{20\,\% typos} \\
  approach             & F1    & acc   & F1    & acc   \\
  \hline
  combined             & 98.52 & 77.09 & 88.99 & 35.02 \\
  combined rob.        & 98.01 & 72.31 & 94.40 & 49.93 \\
  softmax            & 91.57 & 43.57 & 81.36 & 29.90 \\
  softmax rob        & 78.50 & 27.07 & 73.82 & 24.72 \\
  sigmoid             & 97.26 & 69.97 & 86.82 & 36.09 \\
  sigmoid rob.        & 94.68 & 56.84 & 91.70 & 46.62 \\
  beam             & 99.40 & 88.53 & 90.45 & 40.60 \\
  beam rob.        & 99.28 & 86.60 & 96.68 & 65.28 \\
  do nothing       & -         & 11.55 & -         & 11.82 \\
  \hline
 \end{tabular}
 \caption{Average Macro F-scores percentages and sequence accuracies across the benchmarks with the same amount of misspellings.}
 \label{tab:eval-means}
 \end{center}
\end{table}
\fi


\iffalse
We observe that the beam search approach yields the best results on all noise levels.
The iterative approach yields its best results with the combined model, followed by the sigmoidal model.
%The softmax model is the worst of our approaches.
All approaches are able to correct some sequences, which is reflected by the fact that the sequence accuracies are much better than the ones from the do-nothing baseline.

On the benchmarks without misspellings the ordinary models are better than the typo-robust models.
On the benchmarks with misspellings the typo-robust models are better, except for the iterative approach with the softmax model, where the typo-robust model is always worse.
On sequences without misspellings we are able to get average F-scores of above 99\,\% and average sequence accuracies of above 88\,\%.
The problem becomes harder the more misspellings are induced into the sequences.
On the benchmarks with 10\,\% misspellings our best results degrade to above 98\,\% average F-score and 74\,\% average sequence accuracy,
and on the benchmarks with 20\,\% misspellings to above 96\,\% average F-score and 65\,\% average sequence accuracy.

Figure \ref{fig:eval0} shows the F-scores and sequence accuracies for our approaches evaluated on the test sets of the 11 benchmarks without misspellings.
The best approach across all benchmarks is the beam search.
The F-scores of the beam search vary little between the benchmarks, ranging from 98.53\,\% on the benchmark with $p=0.1$ to 99.66\,\% on the benchmark with $p=1$.
The sequence accuracies decrease with an increasing amount of tokenization errors, ranging from 92.56\,\% to 85.72\,\%.
The beam search with the typo-robust model is slightly worse on all benchmarks.
%on average absolute 0.12\,\% worse in F-score and absolute 1.93\,\% worse in sequence accuracy.
The next best approach on the benchmark with $p=0.1$ is the sigmoidal model, whereas the next best approach on the benchmarks with more tokenization errors is the combined model.
All models are better than their typo-robust counterparts on all benchmarks.
The baseline gets exactly those sequences right that do not contain any tokenization errors, which results in sequence accuracies between 4.08\,\% and 30.79\,\%.

Figure \ref{fig:eval01} shows the F-scores and sequence accuracies on the test sets of the 11 benchmarks with a 10\,\% misspelling probability.
The best approach across all benchmarks is the beam search using the typo-robust forward model.
The F-score is rather stable for varying amounts of tokenization errors (minimum 95.48\,\%, maximum 98.86\,\%), whereas the sequence accuracy reduces from 85.53\,\% on the easiest benchmark to 66.10\,\% on the most difficult benchmark.
The typo-robust sigmoidal model and the typo-robust combined model are better than the ordinary models, with the exception of the sigmoidal model for the benchmarks with $0.8 \leq p \leq 1$.
Again, the sigmoidal model is better on benchmarks with few tokenization errors, and the combined model better on benchmarks with many tokenization errors.

Figure \ref{fig:eval02} shows the F-scores and sequence accuracies on the test sets of the 11 benchmarks with a 20\,\% misspelling probability.
The typo-robust beam search gets the best sequence accuracies on all benchmarks,
and the best F-score on all benchmarks except for the benchmark with $p=0.1$, where the iterative procedure with the typo-robust combined model is better.
The typo-robust sigmoidal and combined models are better than the normal models on all benchmarks.

Figure \ref{fig:runtimes} shows the average runtime per sequence on the 11 benchmarks without misspellings.
The runtimes on the benchmarks with misspellings are similar and therefore omitted for brevity.
The runtimes of the iterative approach increase with more tokenization errors, because more iterations are done per sequence.
The runtime of the beam search, on the other hand, is independent of the amount of tokenization errors.
The beam search is the fastest procedure on most of the benchmarks, whereas the sigmoidal iterative approach is fastest when $p \leq 0.2$.
The iterative procedure is slower when the combined model is used, where two models are queried in every iteration.
The sigmoidal model is a little bit faster than the softmax model.
\fi

\iffalse
\begin{figure*}[bt]
 \includegraphics[width=\textwidth]{plots/eval0}
 \caption{F-score and sequence accuracy on the benchmarks without misspellings.}
 \label{fig:eval0}
\end{figure*}

\begin{figure*}[bt]
 \includegraphics[width=\textwidth]{plots/eval01}
 \caption{F-score and sequence accuracy on the benchmarks with a 10\,\% typo probability.}
 \label{fig:eval01}
\end{figure*}

\begin{figure*}[bt]
 \includegraphics[width=\textwidth]{plots/eval02}
 \caption{F-score and sequence accuracy on the benchmarks with a 20\,\% typo probability.}
 \label{fig:eval02}
\end{figure*}

\begin{figure}[bt]
 \begin{center}
  \includegraphics[width=\columnwidth]{plots/t0}
  \caption{Average runtime per sequence on the benchmarks without misspellings.}
  \label{fig:runtimes}
 \end{center}
\end{figure}
\fi




%%%%% APPROACH

\iffalse
\textbf{Bidirectional softmax model.}
An alternative to the combined model is a bidirectional model
that estimates $p_\bi(s | \allowbreak c_b, c_a)$ directly.
It consists of a forward and a backward LSTM cells.
The output of the two cells is concatenated and fed into a dense layer,
which is followed by a softmax output layer as in the unidirectional models.
To estimate the probability $p_\bi(s_i|c_b, c_a)$ of a character $s_i$,
the outputs of the forward cell after processing $s_{i-1}$
and the backward cell after processing $s_{i+1}$ are fed into the dense layer.

The deletion probability is computed as the inverse character probability,
where the character is a space:
$$p_\del(c_b, c_a) = 1 - p_\bi(\msp|c_b, c_a)$$
To estimate insertion probabilities $p_\ins^\bi(s|c_b, c_a)$
between two characters $s_i$ and $s_{i+1}$,
the outputs of the forward cell after $s_{i}$
and the backward cell after $s_{i+1}$ are fed into the dense layer.
%as shown in Figure \ref{subfig:insertion}.
The space insertion probability is retrieved from the estimated insertion probabilities:
$$p_\ins(c_b, c_a) = p_\ins^\bi(\msp|c_b, c_a)\,.$$
This architecture is trained using the categorical crossentropy \cite{Goodfellow} as a loss function.  % \input{figures/bidirectional_lms}
\\\\
\textbf{Bidirectional sigmoidal model.}
The bidirectional softmax model tends to predict high probabilities for space insertions
in words which can be split into two other words,
for example ``however'' into ``how'' and ``ever''.
However, the model must be able to predict the absence of any character between
two context strings to give better estimates of the insertion and deletion probabilities.
Therefore, we introduce another bidirectional model
where the softmax output function is replaced by a sigmoidal output function.
It returns probabilities for each character,
but without the restriction that the probabilities must sum up to 1.
It is therefore able to predict a vector of zeros when no character is
likely to occur between two context strings.
\TODO{mention how you calculate $p_\del$ and $p_\ins$}

This architecture was trained by minimizing the sum of two losses:
the binary crossentropy of the characters in the training sequence
and the binary crossentropy of the predicted insertion probabilities compared with the zero vector.
We call the character training examples the \textit{positive} examples
and the zero-vector training examples the \textit{negative} examples.
An example is given in table \ref{tab:training-examples}.
\fi

\iffalse
\begin{table}[ht]
 \begin{center}
 \begin{tabular}{|l|l|c|}
  \hline
  $c_b$          & $c_a$         & target \\ \hline
                 & reiburg       & F      \\
  F              & eiburg        & r      \\
  Fr             & iburg         & e      \\
  Fre            & burg          & i      \\
  Frei           & urg           & b      \\
  Freib          & rg            & u      \\
  Freibu         & g             & r      \\
  Freibur        &               & g      \\ \hline
                 & Freiburg      & 0      \\
  F              & reiburg       & 0      \\
  Fr             & eiburg        & 0      \\
  Fre            & iburg         & 0      \\
  Frei           & burg          & 0      \\
  Freib          & urg           & 0      \\
  Freibu         & rg            & 0      \\
  Freibur        & g             & 0      \\
  Freiburg       &               & 0      \\
 \hline
 \end{tabular}
 \caption{Positive and negative training examples for the training sequence \textit{``Freiburg''}.
          The 0 denotes the zero vector, i.e. the absence of any character.
          \TODO{Shrink this table or remove it}
          }
 \label{tab:training-examples}
 \end{center}
\end{table}
\fi

\iffalse
%The traceback of $R$ can reconstruct the solution using the recursive function:
%$$TR(w, i) = w_{[i, j^{*})} \oplus \msp \oplus TR(w, j^{*})$$
%where $j^{*}$ is the optimal index for $R(w, i)$. Finally, $TR(S, 0)$ is the
%result of the retokenized text.

% which drops the time complexity
%from $\mathcal{O}(|w|^2)$ to $\mathcal{O}(|w| W)$ on the average case scenario.
%It doesn't improve the worst case scenario where the given text has no spaces.

Finally, since the function $R$ could be not very efficient in terms of time complexity,
we introduce a heuristic of retokenizing only small windows of tokens.
This is based on the assumption that a tokenization error shouldn't affect another
tokenization error which is too distant. Consequently, so retokenize $S$, we first
tokenize it into a sequence $t$ of tokens, then we solve this by introducing a recursive
function $G$, defined by:
$$G(t, i) = \max_{j, i < j \leq i + w - 1, |t|} R(t_i \oplus \cdots \oplus t_{j-1}, 0) + G(t, j)$$
where $w$ is the window size (we chose it to be 5). Then the traceback can be built
recursively by: $$TG(t, i) = TR(t_i \oplus \cdots \oplus t_{j^{*}}, 0) \oplus TG(t, j^{*})$$
where $j^{*}$ is the optimal index for $G(t, i)$.

In conclusion, $S$ can be fixed by tokenizing it into a sequence $t$ of tokens,
then the value $TG(t, 0)$ will be the retokenized string.
\fi


==> sections/evaluations.tex <==
\pdfoutput=1

\def\ptoko{p_{\text{space}}}
\def\ptypo{p_{\text{spell}}}

\subsection{Datasets}\label{sec:evaluation:dataset}

\subsubsection{Wikipedia}

We extracted the articles from the Wikipedia dump of June 20, 2019\footnote{\url{https://dumps.wikimedia.org/enwiki}}
using WikiExtractor \cite{attardi:wiki-extractor}.
The articles were split into sentences with the NLTK sentence segmenter \cite{nltk}.
We did a preprocessing to remove incomplete sentences and sentences containing Markup.
We thus obtain 43,103,197 sequences for training, and 10,000 sequences each for penalty optimization, development and test.

\subsubsection{arXiv}

We used the benchmark generator from \citet{PDFs} to generate
the text from 910,000 articles from arXiv
(parsed from \LaTeX\ files and serving as our ground truth)
as well as the text extracted from the corresponding PDF files
(using \emph{pdftotext} from \citet{pdftotext}).
% and serving as the input for our tokenization repair).
The files were split into paragraphs, which were matched with the ground truth
by searching for a text span that differed from the paragraph only by spaces.
We thus obtain 64,965,651 sequences for training,
and 10,000 sequences each for penalty optimization, development and test.

\subsubsection{ACL anthology corpus}

The ACL corpus is extracted from scientific articles published between 1965 and 2012 \cite{nastase}.
\TODO{This sounds like the ACL corpus is from \cite{nastase}, but that is not true, or is it?}
The publications were scanned and parsed using OCR, and hence have many typical OCR errors.
% This corpus is also used for the evaluation in \citet{nastase}, where they noted that most errors are OCR errors and spurious spaces.
% We could not obtain the ground truth of this dataset.
We manually corrected the tokenization and spelling of 500 sequences as a development set and 500 sequences as a test set, and used the development set for penalty optimization.
% We used the development set as a penalty optimization set.
% We did not train on the ACL corpus because that requires large amounts of text without tokenization errors.

\subsection{Inducing tokenization and spelling errors}\label{sec:evaluation:noise}

To train our models on noisy text, and to create a large synthetic benchmark, we induce tokenization and spelling errors into clean text.

We derive statistics about OCR errors by a comparison of the ACL corpus with a cleaned version\footnote{\url{https://web.eecs.umich.edu/~lahiri/acl_arc.html}, we found the corrections to be incomplete, and therefore do not use the cleaned corpus for training or evaluation, but to derive statistics about typical OCR errors.},
and from the ICDAR 2017 and 2019 OCR postcorrection benchmarks \cite{icdar2017, icdar2019}.
% We compute the character edits between the cleaned and noisy texts.
We define an OCR error as the replacement of zero or more characters in the cleaned text by zero or more characters in the noisy text.
We count the frequency of each OCR error (for example, \ourexample{h} is replaced by \ourexample{il} 7,291 times).

We use our ACL development set to derive statistics about tokenization and spelling error rates.
For each erroneous text span, we compute the number of space insertions and deletions and OCR errors, and divide by the number of characters to get error rates.
The development set contains 187 hyphenation errors and 5,360 tokens which can be hyphenated using \textit{PyHyphen}\footnote{\url{https://pypi.org/project/PyHyphen/}}. This gives a hyphenation probability $p_h = 3.5\%$.

Given a clean sequence, we hyphenate each token with probability $p_h$ using \textit{PyHyphen}.
Each token has a probability of 5.8\% to be the beginning of an erroneous span,
equally as in our development set.
We sample the span length $l$, space insertion and deletion rates and OCR error rates from the collected data points,
and introduce errors into the next $l$ tokens accordingly,
where OCR errors are sampled following their frequency in the ACL and ICDAR datasets.

\subsection{Models training}\label{sec:evaluation:models}

\TODO{Mostafa: we are using the BID ambiguously here, BID in the evaluation section refers to the mix of
UNI and the "bidirectional labelling" model. In the training however, we don't train BID (only in the penalties),
instead we train the individual components UNI and the bidirectional labelling model,
we should resolve this ambiguity. We can simply give the "bidirectional labelling model" a short name like (BIL) or something and use it instead.}
We train four models, using our unidirectional (UNI) and bidirectional (BID) models from Section \ref{sec:approach}
and the combined training data from Wikipedia and arXiv.
We train models on clean text or on noisy text with OCR errors.
For the noisy training, we introduce random OCR errors, which we collected from the ACL and ICDAR datasets, with a uniform probability of 10\% per character, but no tokenization errors.
\\[1mm]
\begin{tabular}{ll}
UNI     & UNI trained on clean text\\
BID     & BID trained on clean text\\
BID+    & BID trained on noisy text\\
The One & BID+ with fixed penalties\\
\end{tabular}\\[1mm]
For each model and benchmark combination, we optimize the penalties $P_\ins$ and $P_\del$
on the penalty optimization set; see Section \ref{sec:evaluation:dataset}.
For ``BID The One'' we set the penalties to the most conservative setting for any of our benchmark
(\TODO{which happens to be ACL with $P_\ins = 7.2$ and $P_\del = 8.3$}),
except when there are no spaces (which is trivial to detect),
in which case $P_\ins = P_\del = 0$.
\TODO{TO DO: training on spelling errors.}

The models were trained for one epoch on a GeForce Titan X GPU,
which took \TODO{43} hours for the unidirectional and \TODO{143} hours for the bidirectional models.
The training was performed using the Adam optimization algorithm \cite{adam}, 
with learning rate 0.001, and mini-batch size 128.
The sequences were cut after 256 characters, while shorter sequences were padded with EOS symbols that got masked in the loss function.
The models are implemented using TensorFlow \cite{tensorflow}.
The UNI Wiki language model has $70.3\,\%$ character accuracy,
$88.9\,\%$ top-5 character accuracy, $1.043$ binary cross-entropy and $87.7\,\%$ space F-score.

\section{Evaluation}

\subsection{Benchmarks}

We evaluate our methods on six benchmarks with different kinds 
of spelling and space errors.
We have also evaluated our approaches on the ICDAR 2017 and 2019 benchmarks,
but do not report this here because of severe issues with the ground truth.%
\footnote{Many corrections were missing and the word order was often significantly changed.
As a minor complication, some of the text uses old language and symbols not encountered in our training data.}

\paragraph{ACL}

The ACL benchmark is made from text fragments from the ACL corpus,
for which we manually created a ground truth.

\paragraph{arXiv OCR}

Since the ground truths of the ACL benchmark are not so many, we create a large similar OCR benchmark
by introducing OCR errors and tokenization errors into the ground truth sequences from the arXiv corpus with the procedure described in section \ref{sec:evaluation:noise}.


\paragraph{arXiv pdftotext}

This benchmark consists of sequences extracted with \textit{pdftotext}, with the corresponding ground truth sequences from the \LaTeX\ source files.

\paragraph{Wikipedia (three variants)}

We create three benchmarks by inducing noise into sentences from Wikipedia.
For one benchmark (\textit{Wiki no\msp}) we remove all spaces.
For another (\textit{Wiki+}) we replace words with misspellings from a pre-defined list\footnote{We collected 228,414 misspellings from \url{https://norvig.com/ngrams/spell-errors.txt}, \url{http://luululu.com/tweet/typo-corpus-r1.txt} and \cite{github-corpus} (94,531 unique misspellings for 33,066 words).}
with 10\% probability, and then introduce tokenization errors uniformly with 0.1 expected error per token.
For the third (\textit{Wiki+ no\msp}) we introduce misspellings and remove all spaces.

%\TODO{Mostafa: I moved the ACL corpus above arXiv, so we can say a motivation regarding the arXiv OCR}


\subsection{Metrics}\label{sec:evaluations:metrics}

\subsubsection{Tokenization repair}

Given a corrupt text $C$, a ground truth text $T$ and a predicted text $P$,
we can frame a repair algorithm as a classifier which predicts a set
of space insertions and deletions that ideally would transform $C$ into $T$.
We use two metrics for the evaluation: F-score and sequence accuracy.

\paragraph{F-score:}\label{sec:evaluation:fscore}

We define $\mathrm{edits}(A, B)$ as the space insertions and deletions that transform $A$ into $B$.
If we let $\mathcal{C} = \mathrm{edits}(C, T)$ be the ground truth edit operations
and $\mathcal{P} = \mathrm{edits}(C, P)$ the predicted edit operations,
the number of true positives is $\mathrm{TP} = |\mathcal{C} \cap \mathcal{P}|$,
the number of false positives is $\mathrm{FP} = |\mathcal{P} \setminus \mathcal{C}|$
and the number of false negatives is $\mathrm{FN} = |\mathcal{C} \setminus \mathcal{P}|$.
% The binary classification metric F-score is the harmonic mean of precision and recall,
% and is computed with:
% The F-score as the harmonic mean of precision and recall is computed with:
The F-score is computed as:
$$F(T, C, P) = \frac{2 \cdot \mathrm{TP}}{2 \cdot \mathrm{TP} + \mathrm{FP} + \mathrm{FN}}$$

\paragraph{Sequence accuracy:}
The sequence accuracy is the fraction of sequences that are corrected completely ($P = T$).
% A sequence is corrected completely if and only if the set of predicted operations
% is exactly equal to the set of ground truth operations for that sequence.

\subsubsection{Spelling correction (F-score)}

We use a word correction F-score as a metric for spelling correction.
We compute the longest common token subsequence of $C$ with $T$ ($C \cap T$), and $P$ with $T$ ($P \cap T$), and define erroneous tokens $E = T \setminus C$, error-free tokens $F = T \cap C$, and correctly predicted tokens $S = P \cap T$.
Then $\mathrm{TP} = |E \cap S|$,
$\mathrm{FP} = |F \setminus S|$
and $\mathrm{FN} = |E \setminus S|$,
and the F-score is computed as above.

We classify each token in $E$ as \textit{tokenization error} if its correction involves only space edits, \textit{spelling error} if only non-space edits, and \textit{mixed} otherwise.

\input{sections/big_table}

\subsection{Main results}\label{sec:evaluations:results}

% Bi-directional are the best on all scenarios, in particular, better than the BS fw from previous work.
Table \ref{tab:eval-results} provides F-scores and sequence accuracies for all our methods on all benchmarks.
We use a beam size of $b=5$ for all beam search approaches; increasing this to $b = 10$ has shown only minimal improvements while doubling the running time.

% Bi-directional models beat all other models and methods
The main takeaway from Table \ref{tab:eval-results} is that the bidirectional models (BID) beat all four baselines by a wide margin on all benchmarks.
It it also significantly better than the unidirectional model (UNI), especially when there are spelling errors.
We remark that it is not obvious that the bidirectional methods are the best,
which might be the reason why previous work used unidirectional methods.
A unidirectional model has the advantage that the tokenization errors are incrementally fixed from left to right, so that the language model predictions can be based on text that is (almost) free from such errors.
However, the text after the current position has not yet been repaired, so that predictions from the other direction are based on text with tokenization errors.
Using these predictions actually \emph{deteriorates} the quality of the unidirectional methods.
Our trick was to combine a unidirectional model that makes use of the space information with a bidirectional model that disregards all space information and thus does not have the aforementioned problem.

The other important takeaways from Table \ref{tab:eval-results} are as follows.
The results for previous work are discussed in Section \ref{sec:evaluations:finer}.

\vspace{1mm}
%Along with that and afterwards, we discuss the other tables (comparison to previous work, error analysis, running time).
\begin{itemize}[parsep=-0.5mm,leftmargin=0mm,itemindent=4mm,topsep=0pt]

% Training on text with spelling errors is essential + doesn't harm on correct text.
\item On the two Wikipedia benchmarks with typos, training on text with spelling errors (Wiki+) is crucial for a good tokenization quality.

% Text with more typos is harder 
\item Tokenization repair is harder when there are \emph{spelling} errors.
This is especially pronounced for the ACL benchmark, which has passages so deformed by OCR errors that there is simply not enough information to reconstruct the correct spacing.
For example, \ourexample{as in the l , a rper above example} or \ourexample{l;h;fl; is, the marginals}.
Still, BID is much better than UNI and also than Google also on this hardest of our benchmarks.

% Text with more space errors is also harder 
\item Tokenization is also harder when there are more \emph{space} errors. 
This is not surprising, yet previous work chose to remove all spaces from the text.
Removing all spaces simplifies the approaches (one only has to predict space insertions, no space deletions),
but the price is much worse results when there were actually only few tokenization errors.
In the table, this corresponds to the two benchmarks with \emph{no \msp},
for which results are significantly worse than for the two benchmarks with \emph{10\,\% \msp}.

% Improvements are hard when most sequences are correct
\item The arXiv benchmark is interesting, because 87.3\% of the sequences have no mistakes.
It is then hard to make corrections in the other 12.7\% without inserting mistakes in the sequences without mistakes.
Indeed, Google is maximally conservative on this benchmark and does not suggest a single correction (hence the zero F-score).
Wordsegment is more bold, with a result that is much worse than doing nothing.
UNI improves slightly over doing nothing, BID improves very significantly.

\item The results for ``BID The One'' are very close to the results of the best models tailored to the respective benchmark (results shown in bold in the table).
This shows that setting the penalties $P_\ins$ and $P_\del$ conservatively does little harm.
It also makes the comparison to tools like Google, which is supposed to work reasonably well for any kind of text, fair.

\end{itemize}

\subsection{Previous work, \DELETE{error analysis,} runtime}\label{sec:evaluations:finer}

\input{sections/small_tables}

The results for the best previous work are shown in Table \ref{tab:related}.
These works did not provide sufficient material so that we could run their methods on our benchmarks.
Instead, we ran our approaches on their benchmarks.
The approach from \cite{doval} is an instance of UNI.
Our implementation of their method has better accuracy; we suspect because we use more training data.
Our method is also better on their benchmark than on our ``Wiki no \msp''; this speaks for their benchmark being easier.
%The results of their method on their benchmark is better than on our benchmark; we suspect because their benchmark (news articles) uses cleaner language and is thus simpler.
The results from \citet{nastase} are very weak in comparison.\footnote{\citet{nastase} report an F-score of 95\%. The explanation for the difference with our result is three-fold: (1) They remove all spaces and then try to restore them (but 95\% restored words is not good when most words had no error initially). (2) They evaluate on the newer documents which have no OCR errors. (3) They make many errors around punctuation, but their word-level evaluation seems not to punish this.}

Methods trained without spelling errors have a strong tendency to split words with a typo because there is no meaningful continuation (e.g., \ourexample{unwnted pregnancies} is wrongly repaired to \ourexample{unw nted pregnancies}) and to wrongly merge misspelled words when they happen to form a correct word (e.g., if \ourexample{as well} is mistyped as \ourexample{s well}, it is wrongly repaired to \ourexample{swell}). \TODO{TODO: find a new example, this one is from an old benchmark.}

We conducted an error analysis on Wikipedia benchmark, the errors consisted of nearly 50\,\% compound words (like \ourexample{offseason})
and compound entity names (Baseball team \ourexample{Waikiki BeachBoys} vs. rock band \ourexample{The Beach Boys}).
20\,\% of the errors are due to foreign words and 20\,\% errors around inconsistent punctuation marks.
The remaining errors were due to abbreviations, measuring unit or unknown alphabet. 
\TODO{Mostafa: I added this paragraph and removed the table, we can remove the next paragraph as well.}
% Comparing BS two-pass with BS bidir
%\TODO{Still up to date?}

% spell check BS
\def\sKB{\,\mathrm{sec\hspace{-0.5mm}/\hspace{-0.5mm}KB}}
The average running time of our tokenization repair, measured on a GeForce Titan X GPU, is $\TODO{X} \sKB$ for UNI and $\TODO{X} \sKB$ for BID.


==> sections/validation_results.tex <==
\newcommand{\msp}{\text{\textvisiblespace}}
\def\field#1#2{\multicolumn{1}{#1}{#2}}  % arguments: #1 position, #2 content
\def\nan#1{\field{c#1}{-}}               % argument:  #1 bounding box to the right
\def\b#1{\textbf{#1}}
\def\sup#1{\textsuperscript{#1}}

\begin{table*}
 \renewcommand{\baselinestretch}{1.2}\small
 \begin{center}
 \begin{tabular}{|l|rrr|rrr||rrr|rrr|}
  \hline
     & \multicolumn{6}{c||}{F-score} & \multicolumn{6}{c|}{sequence accuracy} \\
  \hline
    & \multicolumn{3}{c|}{no typos} & \multicolumn{3}{c||}{10\,\% typos} & \multicolumn{3}{c|}{no typos} & \multicolumn{3}{c|}{10\,\% typos} \\
  approach             & \field{c}{10\,\%} & \field{c}{100\,\%} & \field{c|}{no \msp} & \field{c}{10\,\%} & \field{c}{100\,\%} & \field{c||}{no \msp}& \field{c}{10\,\%} & \field{c}{100\,\%} & \field{c|}{no \msp}& \field{c}{10\,\%} & \field{c}{100\,\%} & \field{c|}{no \msp} \\
  \hline
 %                           F-scores                                                   | sequence accuracies
 %                           no typos                     | with typos                  | no typos                    | with typos
 %                              10 %      100 %     no        10 %      100 %     no        10 %       100 %    no        10 %       100 %    no    
  do nothing                &       - &       - &       - &       - &      -  &       - &   35.63 &    3.16 &    4.17 &   34.76 &    2.86 &    4.17 \\
  greedy                    &   85.30 &   56.20 &   20.30 &   68.17 &   53.46 &   19.70 &   77.23 &    9.92 &   12.90 &   46.51 &    8.41 &   11.16 \\
  bigram DP                 &   91.35 &   99.07 &   99.03 &   67.58 &   95.41 &   95.24 &   86.06 &   86.06 &   86.06 &   45.43 &   45.43 &   45.43 \\
  wordsegment               &   58.23 &   93.37 &   92.84 &   45.71 &   89.35 &   88.39 &   41.28 &   41.28 &   41.28 &   22.01 &   22.01 &   22.01 \\
  Google \sup{1}            &   89.78 &   65.43 &   18.40 &   82.95 &   53.14 &   15.14 &   82.00 &   15.00 &   15.00 &   73.00 &   10.00 &   13.00 \\
  \hline
  bidirectional             &   98.86 &   99.70 &   99.66 &   93.35 &   98.26 &   98.03 &   96.98 &   93.51 &   93.35 &   83.67 &   68.93 &   68.15 \\
  bidir. robust             &   98.52 &   99.64 &   99.58 &   97.45 &   99.28 &   99.19 &   96.24 &   92.35 &   92.01 &   93.42 &   84.94 &   84.17 \\
  \hdashline
  BS fw                     &   98.58 &   99.64 &   99.57 &   93.99 &   97.93 &   97.51 &   96.38 &   92.64 &   91.73 &   85.52 &   67.65 &   65.31 \\
  BS bw                     &   98.49 &   99.63 &   99.56 &   93.33 &   97.81 &   97.46 &   96.16 &   92.56 &   91.99 &   83.94 &   66.60 &   64.54 \\
  BS fw robust              &   98.42 &   99.57 &   99.50 &   98.00 &   99.32 &   99.19 &   96.05 &   91.58 &   91.09 &   95.04 &   87.20 &   86.27 \\
  BS bw robust              &   98.49 &   99.57 &   99.49 &   98.05 &   99.30 &   99.17 &   96.25 &   91.82 &   91.15 &   95.16 &   87.55 &   86.38 \\
  \hdashline
  2-pass BS                 &   98.63 &   99.69 &   99.62 &   94.06 &   98.17 &   97.83 &   96.51 &   93.66 &   92.73 &   85.59 &   70.70 &   68.85 \\
  2-pass BS robust          &   98.47 &   99.62 &   99.55 &   98.13 &   99.43 &   99.34 &   96.21 &   92.65 &   92.13 &   95.38 &   89.23 &   88.60 \\
  \hdashline
  BS bidir                  &   98.97 &   99.73 &   99.69 &   95.76 &   98.64 &   98.41 &   97.36 &   94.55 &   94.23 &   89.37 &   75.21 &   73.32 \\
  BS bidir robust           &   98.83 &   99.70 &   99.66 &   98.48 &   99.55 &   99.46 &   97.01 &   93.88 &   93.52 &   96.18 &   90.83 &   90.04 \\
  \hline
 \end{tabular}
 \caption{F-scores and sequence accuracy percentages for all models and all benchmarks. The benchmarks either contain
     no typos or 10\% chance of introducing a typo. The tokenization errors either have $p$ as $0.1$, $1.0$ or
     all spaces removed.  The F-scores are micro-averaged across the \emph{development} set.
     The difference of the sequence accuracy of the best approach compared with all other approaches is statistically strongly significant ($p < 0.01$ with a paired two-sided randomization test) \hspace{7mm} \sup{1} Google's tokenization repair was manually evaluated on 100 development sequences.
     }
 \label{tab:eval-results}
     \vspace{-0.5cm}
 \end{center}
\end{table*}


